LooGLE: Can Long-Context Language Models Understand Long Contexts?

Large language models (LLMs), despite their impressive performance in various language tasks, are typically limited to processing texts within context-window size. This limitation has spurred significant research efforts to enhance LLMs' long-context understanding with high-quality long-sequence benchmarks. However, prior datasets in this regard suffer from shortcomings, such as short context length compared to the context window of modern LLMs; outdated documents that have data leakage problems; and an emphasis on short dependency tasks rather than long dependency tasks. In this paper, we present LooGLE, a Long Context Generic Language Evaluation benchmark for LLMs' long context understanding. LooGLE features relatively new documents post-2022, with over 24,000 tokens per document and 6,000 newly generated questions spanning diverse domains. Human annotators meticulously crafted more than 1,100 high-quality question-answer pairs to meet the long dependency requirements. These pairs underwent thorough cross-validation, yielding the most precise assessment of LLMs' long dependency capabilities. The evaluation of eight state-of-the-art LLMs on LooGLE revealed key findings: (i) commercial models outperformed open-sourced models; (ii) LLMs excelled in short dependency tasks like short question-answering and cloze tasks but struggled with more intricate long dependency tasks; (iii) in-context learning and chaining thoughts offered only marginal improvements; (iv) retrieval-based techniques demonstrated substantial benefits for short question-answering, while strategies for extending context window length had limited impact on long context understanding. As such, LooGLE not only provides a systematic and comprehensive evaluation schema on long-context LLMs, but also sheds light on future development of enhanced models towards "true long-context understanding".

==> tables/comparision_with_other_bench.tex <==
\begin{table}[t!]
    % \vspace{-10pt}
    \centering
    \caption{Comparison with other long-context benchmarks.}
    \label{tab:benchmark_comparison}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{llccccccccc}
    \toprule
        \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Avg. Words}} & \multirow{2}{*}{\textbf{\# of Docs.}} & \multirow{2}{*}{\textbf{\# of Ques.}} & \multirow{2}{*}{\textbf{Manually Label}} & \multicolumn{5}{c}{\textbf{Long Dependency Tasks}}\\ \cmidrule{7-11}
        &  & & & & Summarization & Info. Retrieval & Timeline Reorder & Computation & Doc QA \\  \midrule
        Zero Scrolls~\citep{shaham2023zeroscrolls} &  & 10,392 & - & 4,378 & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark\\
        Long Bench~\citep{bai2023longbench} & & 8,120 & - & 4,750 & 350 & \cmark & \cmark$^*$ & \xmark & \cmark$^*$ & \cmark\\
        L-Eval~\citep{an2023leval} & & 8,008 & 411 & 2,043 & 2,043$^\dagger$ & \cmark & \cmark & \xmark & \xmark & \cmark\\ \midrule
        \dataset~(Ours) & 16,375 & 778 & 6,467 & 1,120 & \cmark & \cmark &\cmark &\cmark &\cmark  
        \\
    \bottomrule
    \multicolumn{11}{l}{\footnotesize $^*$ The task is created in a synthetic manner.} \\
    \multicolumn{11}{l}{\footnotesize $^\dagger$ The questions are re-labelled from original data.} \\

    \end{tabular}
}
\end{table}

==> tables/dataset_intro_bk.tex <==
\begin{table}[t]
\vspace{-30pt}
\caption{Statistics of LooGLE}
\label{tab:benchmark}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccccc}
\toprule
{\textbf{Dataset}} & 
{\textbf{Category}} &
{\textbf{No. Documents}} &
{\textbf{Avg. Words}} &
{\textbf{Avg. Tokens}} &
{\textbf{Task}} & 
{\textbf{Subtask}} & 
{\textbf{No. Questions}}  \\ 
    % \textbf{} &
    % \textbf{ }  &
    % \textbf{ }  &
    % \textbf{ }  &
    % \textbf{} & \\
    \midrule

    
\multirow{2}{*}{\makecell[c]{\begin{tabular}[c]{@{}c@{}}arXiv papers  \end{tabular}} }                                                                  & {\makecell[c]{Physics, Math, \\Finance, Statistics, \\Biology, Economics, \\Computer Science, etc.}}                                             & 516                  & 16,988                  & 20,887                           & Summarization                 & —                          & 516  \\
\midrule
\multirow{5}{*}{\makecell[c]{\begin{tabular}[c]{@{}c@{}}Wikipedia \\ pages\end{tabular}}}      & \multirow{3}{*}{\makecell[c]{Events, History, \\Famous person, Sports, \\Politics, Arts,\\ Awards, Military,\\ Medical, etc.}} & \multirow{4}{*}{\makecell[c]{105}} & \multirow{4}{*}{17,604} & \multirow{4}{*}{21,017} & short dependency QA                 & —                          & 1,951 \\
                                                                                 &                                                                                                                            &                      &                        &                                 &                                & \makecell[l]{Comprehension \& reasoning} & 152  \\
                                                                                 &                                                                                                                            &                      &                        &                                 &                 & \makecell[l]{Multiple  information retrieval}         & 158  \\
                                                                                 &                                                                                                                            &                      &                        &                                 &    {long dependency QA}                            & \makecell[l]{Timeline reorder}                   & 83   \\
                                                                                 &                                                                                                                            &                      &                        &                                 &                               & \makecell[l]{Computation}                & 66   \\
\midrule
\multirow{5}{*}{\makecell[c]{\begin{tabular}[c]{@{}c@{}}Movie and \\ TV scripts\end{tabular}}} & \multirow{4}{*}{\makecell[c]{Action, Adventure, \\Comedy, Drama, \\Fantasy, Horror, \\Mystery, Romantic, \\Science Fiction, Thriller}}          & \multirow{4}{*}{\makecell[c]{155}} & \multirow{4}{*}{\makecell[c]{28,483}} & \multirow{4}{*}{\makecell[c]{36,412}}          & short dependency Cloze              & —                          & 2,880 \\
                                                                                 &                                                                                                                            &                      &                        &                                 &                               &\makecell[l] {Comprehension \& reasoning} & 254  \\
                                                                                 &                                                                                                                            &                      &                        &                                 &                &\makecell[l] {Multiple information retrieval}         & 222  \\
                                                                                 &                                                                                                                            &                      &                        &                                 &    {long dependency QA}                            & \makecell[l]{Timeline reorder}                  & 132  \\
                                                                                 &                                                                                                                              &                      &                        &                               &                               & \makecell[l]{Computation}                & 34   \\ 
\midrule
Total                                                                                                  &                                                                                                                                                 & 776                                       & 19,367                                       & 24,005                                       &                                                    &                                                 & 6,448    \\                                                                                                                                                                 
                                                                                 
                                                                                 \bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table}

==> tables/dataset_intro_bk1.tex <==
\begin{table*}[t!]
% \vspace{-10pt}
\renewcommand{\arraystretch}{0.7}
\setlength{\tabcolsep}{2pt}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccccccc}
\toprule
{\textbf{Dataset}} & 
{\textbf{Category}} &
{\textbf{No. Docs}} &
{\textbf{Avg. Words}} &
{\textbf{Max. Words}} &
{\textbf{Min. Words}} &
{\textbf{Avg. Tokens}} &
{\textbf{Task}} & 
{\textbf{Subtask}} & 
{\textbf{No. Questions}}  \\ 
    % \textbf{} &
    % \textbf{ }  &
    % \textbf{ }  &
    % \textbf{ }  &
    % \textbf{} & \\
    \midrule

    
\multirow{2}{*}{\makecell[c]{\begin{tabular}[c]{@{}c@{}}arXiv papers  \end{tabular}} }                                                                  & {\makecell[c]{Physics, Math, \\Finance, Statistics, \\Biology, Economics, \\Computer Science, etc.}}                                             & 516                  & 16,988     & 197,977   & 10,204               & 20,887                           & Summarization                 & —                          & 516  \\
\midrule
\multirow{5}{*}{\makecell[c]{\begin{tabular}[c]{@{}c@{}}Wikipedia \\ pages\end{tabular}}}      & \multirow{3}{*}{\makecell[c]{Events, History, \\Famous person, Sports, \\Politics, Arts,\\ Awards, Military,\\ Medical, etc.}} & \multirow{4}{*}{\makecell[c]{105}} & \multirow{4}{*}{17,604} & \multirow{4}{*}{46,250} & \multirow{4}{*}{11,285} & \multirow{4}{*}{21,017} & short dependency QA                 & —                          & 1,951 \\
                                                                                 &                                                                                                                            &                      &                        &                                 &                  &&              & \makecell[c]{CR} & 152  \\
                                                                                 &                                                                                                                            &                      &                        &                                 &              &&   & \makecell[c]{MR}         & 158  \\
                                                                                 &                                                                                                                            &                      &                        &                               &&  &    {long dependency QA}                            & \makecell[c]{TR}                   & 83   \\
                                                                                 &                                                                                                                            &                      &                        &                                 &                           &&    & \makecell[c]{CAL}                & 66   \\
\midrule
\multirow{5}{*}{\makecell[c]{\begin{tabular}[c]{@{}c@{}}Movie and \\ TV scripts\end{tabular}}} & \multirow{4}{*}{\makecell[c]{Action, Adventure, \\Comedy, Drama, \\Fantasy, Horror, \\Mystery, Romantic, \\Science Fiction, Thriller}}          & \multirow{4}{*}{\makecell[c]{155}} & \multirow{4}{*}{\makecell[c]{28,483}}  & \multirow{4}{*}{\makecell[c]{62,752}}  & \multirow{4}{*}{\makecell[c]{11,089}} & \multirow{4}{*}{\makecell[c]{36,412}}          & short dependency Cloze              & —                          & 2,880 \\
                                                                                 &                                                                                                                            &                      &                        &                                 &                        &&       &\makecell[c] {CR} & 254  \\
                                                                                 &                                                                                                                            &                      &                        &                                 &             &&   &\makecell[c] {MR}         & 222  \\
                                                                                 &                                                                                                                            &                      &                        &                              &&   &    {long dependency QA}                            & \makecell[c]{TR}                  & 132  \\
                                                                                 &                                                                                                                              &                      &                        &                               &                         &&      & \makecell[c]{CAL}                & 34   \\ 
\midrule
Total                                                                                                  &                                                                                                                                                 & 776                                       & 19,367     & 197,977  & 10,204                                   & 24,005                                       &                                                    &                                                 & 6,448    \\                                                                                                                                                                 
                                                                                 
                                                                                 \bottomrule
\\                                                                                 
\multicolumn{8}{l}{CR refers to Comprehension \& Reasoning, MR refers to Multi-source Retrieval, TR refers to Timeline Reorder. CAL refers to Calculation.}
\end{tabular}
}
\caption{\label{tab:benchmark}Statistics of LooGLE}
% \vspace{-10pt}
\end{table*}
